Auto-RT: Automatic Jailbreak Strategy Exploration for Red-Teaming Large Language Models

Automated red-teaming has become a crucial approach for uncovering vulnerabilities in large language models (LLMs). However, most existing methods focus on isolated safety flaws, limiting their ability to adapt to dynamic defenses and uncover complex vulnerabilities efficiently. To address this challenge, we propose Auto-RT, a reinforcement learning framework that automatically explores and optimizes complex attack strategies to effectively uncover security vulnerabilities through malicious queries. Specifically, we introduce two key mechanisms to reduce exploration complexity and improve strategy optimization: 1) Early-terminated Exploration, which accelerate exploration by focusing on high-potential attack strategies; and 2) Progressive Reward Tracking algorithm with intermediate downgrade models, which dynamically refine the search trajectory toward successful vulnerability exploitation. Extensive experiments across diverse LLMs demonstrate that, by significantly improving exploration efficiency and automatically optimizing attack strategies, Auto-RT detects a boarder range of vulnerabilities, achieving a faster detection speed and 16.63\% higher success rates compared to existing methods.

==> figures/fig_fs_il.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{resources/iml_qwen15_14.pdf}
        \vspace{0.5em}
        (a) Few-Shot
    \end{minipage}
    % \hspace{0.05\linewidth}
    \begin{minipage}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{resources/iml_qwen15_14.pdf}
        \vspace{0.5em}
        (b)  Imitate Learning
    \end{minipage}
    \caption{TODO}
    \label{fig:fs_il}
\end{figure}


==> sections/limitation.tex <==
\section{Limitations}
Firstly, our work focuses solely on single-turn dialogue attack scenarios. Recent studies have shown that safety-aligned language models exhibit more significant security risks in multi-turn dialogues and agent applications compared to single-turn interactions. Future research could explore these more complex scenarios to uncover additional vulnerabilities. Secondly, due to computational resource constraints, we optimized only the strategy generation model without specifically enhancing the strategy rephrasing model. Optimizing both models together could help identify a broader range of security risks.

==> tables/div-ca.tex <==
% Table generated by Excel2LaTeX from sheet '16-dive-ft'
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{lrrrrr}
    \toprule
          & \multicolumn{1}{l}{Imitate Learning} & \multicolumn{1}{l}{Few-Shot} & \multicolumn{1}{l}{AutoDAN} & \multicolumn{1}{l}{RL} & \multicolumn{1}{l}{Meta-RT} \\
    \midrule
    Vicuna 7B & 5.2   & 6.3   & 7.15  & 20.1  & 46.80  \\
    Vicuna 13B & 4.5   & 8.1   & 1.20  & 21.03 & 56.33  \\
    Llama 2 7B Chat & 2.7   & 3.5   & 0.05  & 0.88  & 12.98  \\
    Llama 2 13B Chat & 3     & 4.2   & 0.75  & 1.15  & 10.85  \\
    Llama 3 8B Instruct & 6.4   & 7     & 11.35  & 7.5   & 15.00  \\
    Mistral 7B Instruct & 9.8   & 12.3  & 35.70  & 28.48 & 48.68  \\
    Yi 6B Chat & 12.1  & 14.6  & 50.35  & 31.45 & 47.25  \\
    Yi 9B Chat & 13    & 15    & 43.00  & 22.6  & 48.90  \\
    Gemma 2 2b Instruct & 3.5   & 5.1   & 4.10  & 3.43  & 47.93  \\
    Gemma 2 9b Instruct & 2.2   & 3.8   & 43.30  & 30.2  & 48.10  \\
    R2D2  & 8.9   & 10.4  & 43.95  & 4.33  & 15.43  \\
    Qwen 1.5 4B Chat & 4.2   & 5.5   & 4.95  & 12.88 & 45.58  \\
    Qwen 1.5 7B Chat & 6.8   & 8     & 10.90  & 25.95 & 34.25  \\
    Qwen 1.5 14B Chat & 5     & 6.9   & 0.55  & 16.4  & 43.40  \\
    Qwen 2.5 3B Chat & 3.8   & 5.2   & 4.05  & 17.25 & 47.85  \\
    Qwen 2.5 14B Chat & 7.5   & 9.1   & 24.8  & 12.38 & 41.78  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> tables/div-sem.tex <==
% Table generated by Excel2LaTeX from sheet '16-dive-sem'
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{lrrrrr}
    \toprule
    Model & \multicolumn{1}{l}{Imitate Learning} & \multicolumn{1}{l}{Few-Shot} & \multicolumn{1}{l}{AutoDAN} & \multicolumn{1}{l}{RL} & \multicolumn{1}{l}{Meta-RT} \\
    \midrule
    Vicuna 7B & 0.864  & 0.702 & 0.966  & 0.641 & 0.57 \\
    Vicuna 13B & 0.934  & 0.768 & 0.995  & 0.505 & 0.504 \\
    Llama 2 7B Chat & 0.900  & 0.737 & 0.862  & 0.536 & 0.456 \\
    Llama 2 13B Chat & 0.854  & 0.651 & 0.862  & 0.543 & 0.561 \\
    Llama 3 8B Instruct & 0.938  & 0.672 & 0.844  & 0.638 & 0.453 \\
    Mistral 7B Instruct & 0.881  & 0.758 & 0.878  & 0.506 & 0.5 \\
    Yi 6B Chat & 0.903  & 0.802 & 0.893  & 0.502 & 0.476 \\
    Yi 9B Chat & 0.914  & 0.801 & 0.899  & 0.568 & 0.592 \\
    Gemma 2 2b Instruct & 0.850  & 0.812 & 0.857  & 0.516 & 0.455 \\
    Gemma 2 9b Instruct & 0.817  & 0.707 & 0.900  & 0.624 & 0.525 \\
    R2D2  & 0.820  & 0.708 & 0.850  & 0.591 & 0.495 \\
    Qwen 1.5 4B Chat & 0.865  & 0.646 & 0.972  & 0.587 & 0.575 \\
    Qwen 1.5 7B Chat & 0.888  & 0.717 & 0.850  & 0.572 & 0.515 \\
    Qwen 1.5 14B Chat & 0.876  & 0.724 & 0.850  & 0.568 & 0.527 \\
    Qwen 2.5 3B Chat & 0.830  & 0.705 & 0.852  & 0.58  & 0.576 \\
    Qwen 2.5 14B Chat & 0.836  & 0.735 & 0.839  & 0.641 & 0.457 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> tables/dive.tex <==
% Table generated by Excel2LaTeX from sheet '16-dive-ft'
\begin{table*}[t]
  \centering
  \renewcommand{\arraystretch}{.9} 
  \newcolumntype{C}{>{\centering\arraybackslash}p{2cm}} 
  \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
          & \multicolumn{2}{C}{IL} & \multicolumn{2}{C}{FS} & \multicolumn{2}{C}{AD} & \multicolumn{2}{C}{RL} & \multicolumn{2}{C}{\our{}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}         & \multicolumn{1}{c}{\textbf{DeD} \uparrow} & \multicolumn{1}{c}{\textbf{SeD} \downarrow} & \multicolumn{1}{c}{\textbf{DeD} \uparrow} & \multicolumn{1}{c}{\textbf{SeD} \downarrow} & \multicolumn{1}{c}{\textbf{DeD} \uparrow} & \multicolumn{1}{c}{\textbf{SeD} \downarrow} & \multicolumn{1}{c}{\textbf{DeD} \uparrow} & \multicolumn{1}{c}{\textbf{SeD} \downarrow} & \multicolumn{1}{c}{\textbf{DeD} \uparrow} & \multicolumn{1}{c}{\textbf{SeD} \downarrow} \\
    \midrule
    Vicuna 7B & 5.24  & 0.86  & 6.30  & 0.70  & 7.15  & 0.97  & 20.10  & 0.64  & \textbf{46.80}  & \textbf{0.57}  \\
    Vicuna 13B & 4.55  & 0.93  & 8.15  & 0.77  & 1.20  & 1.00  & 21.03  & 0.51  & \textbf{56.33}  & \textbf{0.50}  \\
    Llama 2 7B Chat & 2.70  & 0.90  & 3.55  & 0.74  & 0.05  & 0.86  & 0.88  & 0.54  & \textbf{12.98}  & \textbf{0.46}  \\
    Llama 2 13B Chat & 3.03  & 0.85  & 4.20  & 0.65  & 0.75  & 0.86  & 1.15  & \textbf{0.54}  & \textbf{10.85}  & 0.56  \\
    Llama 3 8B Instruct & 6.40  & 0.94  & 7.00  & 0.67  & 11.35  & 0.84  & 7.50  & 0.64  & \textbf{15.00}  & \textbf{0.45}  \\
    Mistral 7B Instruct & 9.80  & 0.88  & 12.35  & 0.76  & 35.70  & 0.88  & 28.48  & 0.51  & \textbf{48.68}  & \textbf{0.50}  \\
    Yi 6B Chat & 12.18  & 0.90  & 14.60  & 0.80  & \textbf{50.35}  & 0.89  & 31.45  & 0.50  & 47.25  & \textbf{0.48}  \\
    Yi 9B Chat & 13.05  & 0.91  & 15.00  & 0.80  & 43.00  & 0.90  & 22.60  & \textbf{0.57}  & \textbf{48.90}  & 0.59  \\
    Gemma 2 2b Instruct & 3.53  & 0.85  & 5.15  & 0.81  & 4.10  & 0.86  & 3.43  & 0.52  & \textbf{47.93}  & \textbf{0.46}  \\
    Gemma 2 9b Instruct & 2.28  & 0.82  & 3.80  & 0.71  & 43.30  & 0.90  & 30.20  & 0.62  & \textbf{48.10}  & \textbf{0.53}  \\
    R2D2  & 8.95  & 0.82  & 10.45  & 0.71  & 43.95  & 0.85  & 4.33  & 0.59  & \textbf{41.78}  & \textbf{0.50}  \\
    Qwen 1.5 4B Chat & 4.20  & 0.87  & 5.50  & 0.65  & 4.95  & 0.97  & 12.88  & 0.59  & \textbf{45.58}  & \textbf{0.58}  \\
    Qwen 1.5 7B Chat & 6.80  & 0.89  & 8.00  & 0.72  & 10.90  & 0.85  & 25.95  & 0.57  & \textbf{34.25}  & \textbf{0.52}  \\
    Qwen 1.5 14B Chat & 5.05  & 0.88  & 6.95  & 0.72  & 0.55  & 0.85  & 16.40  & 0.57  & \textbf{43.40}  & \textbf{0.53}  \\
    Qwen 2.5 3B Chat & 3.80  & 0.83  & 5.20  & 0.71  & 4.05  & 0.85  & 17.25  & \textbf{0.58}  & \textbf{47.85}  & \textbf{0.58}  \\
    Qwen 2.5 14B Chat & 7.50  & 0.84  & 9.10  & 0.74  & 24.80  & 0.84  & 12.38  & 0.64  & \textbf{15.43}  & \textbf{0.46}  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:dive}%
  \caption{Add caption}
\end{table*}%


==> tables/effective.tex <==
% % Table generated by Excel2LaTeX from sheet '16-effective'
% \begin{table*}[t!]
%   \centering
%   \resizebox{\linewidth}{!}{
%     \begin{tabular}{lrrrrrrrr}
%     \toprule
%           & \multicolumn{1}{l}{Direct Attack} & \multicolumn{1}{l}{Few-Shot} & \multicolumn{1}{l}{Imitate Learning} & \multicolumn{1}{l}{AutoDAN} & \multicolumn{1}{l}{Human} & \multicolumn{1}{l}{Past-Time} & \multicolumn{1}{l}{RL} & \multicolumn{1}{l}{Meta-RT} \\
%     \midrule
%     Vicuna 7B & 24.80  & 29.58  & 36.9  & \textbf{81.85 } & 44.69  & 24.00  & 31.95  & 56.40  \\
%     Vicuna 13B & 16.60  & 20.80  & 36.08 & \textbf{83.00 } & 44.69  & 23.00  & 17.80  & 55.35  \\
%     Llama 2 7B Chat & 0.45  & 6.84  & 6.67  & 0.99  & 5.44  & 2.00  & 0.50  & \textbf{13.50 } \\
%     Llama 2 13B Chat & 1.30  & 5.88  & 6.8   & \textbf{17.82 } & 5.81  & 0.00  & 2.05  & 11.00  \\
%     Llama 3 8B Instruct & 3.20  & 9.42  & 7.18  & 0.02  & 3.38  & 6.00  & 14.55  & \textbf{15.00 } \\
%     Mistral 7B Instruct & 48.50  & 51.54  & 54.88 & \textbf{83.06 } & 71.60  & 22.00  & 44.20  & 52.65  \\
%     Yi 6B Chat & 13.45  & 36.00  & 42.29 & \textbf{75.64 } & 53.00  & 24.00  & 33.80  & 52.50  \\
%     Yi 9B Chat & 16.75  & 28.06  & 34.23 & \textbf{71.10 } & 54.69  & 19.00  & 39.75  & 49.20  \\
%     Gemma 2 2b Instruct & 2.05  & 5.64  & 7.49  & \textbf{76.02 } & 40.92  & 9.00  & 6.15  & 48.15  \\
%     Gemma 2 9b Instruct & 1.55  & 3.74  & 6.63  & \textbf{68.06 } & 51.77  & 8.00  & 44.85  & 44.80  \\
%     R2D2  & 1.70  & 27.18  & 24.24 & \textbf{15.59 } & 7.75  & 0.00  & 8.60  & 12.45  \\
%     Qwen 1.5 4B Chat & 12.50  & 27.24  & 18.52 & \textbf{80.60 } & 42.92  & 6.00  & 17.45  & 51.30  \\
%     Qwen 1.5 7B Chat & 21.70  & 23.80  & 18.82 & \textbf{80.87 } & 60.07  & 14.00  & 32.60  & 49.85  \\
%     Qwen 1.5 14B Chat & 17.20  & 18.78  & 23.82 & \textbf{71.74 } & 55.06  & 21.00  & 17.75  & 42.50  \\
%     Qwen 2.5 3B Chat & 16.30  & 30.94  & 38.3  & \textbf{64.48 } & 43.81  & 18.00  & 20.35  & 42.20  \\
%     Qwen 2.5 14B Chat & 3.80  & 15.42  & 9.38  & 12.83  & 11.95  & 22.00  & 15.65  & \textbf{17.15 } \\
%     \bottomrule
%     \end{tabular}%
%     }
%   \caption{Add caption}
%   \label{tab:effective}%
% \end{table*}%


% Table generated by Excel2LaTeX from sheet '16-effective'
% \begin{table*}[t]
%   \centering
%   \resizebox{\linewidth}{!}{

%     \begin{tabular}{lrrrrrrrr}
%     \toprule
%     \multirow{2}[4]{*}{} & \multicolumn{1}{c}{\multirow{2}[4]{*}{Direct Attack}} & \multicolumn{3}{c}{Human Based} & \multicolumn{3}{c}{Machine Based} & \multicolumn{1}{c}{\multirow{2}[4]{*}{Meta-RT}} \\
% \cmidrule{3-8}          &       & \multicolumn{1}{l}{AutoDAN} & \multicolumn{1}{l}{Human} & \multicolumn{1}{l}{Past-Time} & \multicolumn{1}{l}{Few-Shot} & \multicolumn{1}{l}{Imitate Learning} & \multicolumn{1}{l}{RL} &  \\
%     \midrule
%     Vicuna 7B & 24.80  & \textbf{81.85 } & 44.69  & 24.00  & 29.58  & 36.90  & 31.95  & 56.40  \\
%     Vicuna 13B & 16.60  & \textbf{83.00 } & 44.69  & 23.00  & 20.80  & 36.08  & 17.80  & 55.35  \\
%     Llama 2 7B Chat & 0.45  & 0.99  & 5.44  & 2.00  & 6.84  & 6.67  & 0.50  & \textbf{13.50 } \\
%     Llama 2 13B Chat & 1.30  & \textbf{17.82 } & 5.81  & 0.00  & 5.88  & 6.80  & 2.05  & 11.00  \\
%     Llama 3 8B Instruct & 3.20  & 0.02  & 3.38  & 6.00  & 9.42  & 7.18  & 14.55  & \textbf{15.00 } \\
%     Mistral 7B Instruct & 48.50  & \textbf{83.06 } & 71.60  & 22.00  & 51.54  & 54.88  & 44.20  & 52.65  \\
%     Yi 6B Chat & 13.45  & \textbf{75.64 } & 53.00  & 24.00  & 36.00  & 42.29  & 33.80  & 52.50  \\
%     Yi 9B Chat & 16.75  & \textbf{71.10 } & 54.69  & 19.00  & 28.06  & 34.23  & 39.75  & 49.20  \\
%     Gemma 2 2b Instruct & 2.05  & \textbf{76.02 } & 40.92  & 9.00  & 5.64  & 7.49  & 6.15  & 48.15  \\
%     Gemma 2 9b Instruct & 1.55  & \textbf{68.06 } & 51.77  & 8.00  & 3.74  & 6.63  & 44.85  & 44.80  \\
%     R2D2  & 1.70  & \textbf{15.59 } & 7.75  & 0.00  & 27.18  & 24.24  & 8.60  & 12.45  \\
%     Qwen 1.5 4B Chat & 12.50  & \textbf{80.60 } & 42.92  & 6.00  & 27.24  & 18.52  & 17.45  & 51.30  \\
%     Qwen 1.5 7B Chat & 21.70  & \textbf{80.87 } & 60.07  & 14.00  & 23.80  & 18.82  & 32.60  & 49.85  \\
%     Qwen 1.5 14B Chat & 17.20  & \textbf{71.74 } & 55.06  & 21.00  & 18.78  & 23.82  & 17.75  & 42.50  \\
%     Qwen 2.5 3B Chat & 16.30  & \textbf{64.48 } & 43.81  & 18.00  & 30.94  & 38.30  & 20.35  & 42.20  \\
%     Qwen 2.5 14B Chat & 3.80  & 12.83  & 11.95  & 22.00  & 15.42  & 9.38  & 15.65  & \textbf{17.15 } \\
%     \bottomrule
%     \end{tabular}%
%   }
%   \label{tab:effective}%
%   \caption{Add caption}
% \end{table*}%

\begin{table*}[t]
  \centering
  \newcolumntype{C}{>{\centering\arraybackslash}p{3em}} 
  \renewcommand{\arraystretch}{.9} 

  \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{ASR_{tst}}\uparrow}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{Direct Attack}} & \multicolumn{3}{c}{Human Based} & \multicolumn{3}{c}{Machine Based} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\our{}}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
          &       & \multicolumn{1}{C}{AD} & \multicolumn{1}{C}{HT} & \multicolumn{1}{C}{PT} & \multicolumn{1}{C}{FS} & \multicolumn{1}{C}{IL} & \multicolumn{1}{C}{RL} &  \\
    \midrule
    Vicuna 7B & 24.80  & \textbf{81.85 } & 44.69  & 24.00  & 29.58  & 36.90  & 31.95  & 56.40  \\
    Vicuna 13B & 16.60  & \textbf{83.00 } & 44.69  & 23.00  & 20.80  & 36.08  & 17.80  & 55.35  \\
    Llama 2 7B Chat & 0.45  & 0.99  & 5.44  & 2.00  & 6.84  & 6.67  & 0.50  & \textbf{13.50 } \\
    Llama 2 13B Chat & 1.30  & \textbf{17.82 } & 5.81  & 0.00  & 5.88  & 6.80  & 2.05  & 11.00  \\
    Llama 3 8B Instruct & 3.20  & 0.02  & 3.38  & 6.00  & 9.42  & 7.18  & 14.55  & \textbf{15.00 } \\
    Mistral 7B Instruct & 48.50  & \textbf{83.06 } & 71.60  & 22.00  & 51.54  & 54.88  & 44.20  & 52.65  \\
    Yi 6B Chat & 13.45  & \textbf{75.64 } & 53.00  & 24.00  & 36.00  & 42.29  & 33.80  & 52.50  \\
    Yi 9B Chat & 16.75  & \textbf{71.10 } & 54.69  & 19.00  & 28.06  & 34.23  & 39.75  & 49.20  \\
    Gemma 2 2b Instruct & 2.05  & \textbf{76.02 } & 40.92  & 9.00  & 5.64  & 7.49  & 6.15  & 48.15  \\
    Gemma 2 9b Instruct & 1.55  & \textbf{68.06 } & 51.77  & 8.00  & 3.74  & 6.63  & 44.85  & 44.80  \\
    R2D2  & 1.70  & \textbf{15.59 } & 7.75  & 0.00  & 27.18  & 24.24  & 8.60  & 12.45  \\
    Qwen 1.5 4B Chat & 12.50  & \textbf{80.60 } & 42.92  & 6.00  & 27.24  & 18.52  & 17.45  & 51.30  \\
    Qwen 1.5 7B Chat & 21.70  & \textbf{80.87 } & 60.07  & 14.00  & 23.80  & 18.82  & 32.60  & 49.85  \\
    Qwen 1.5 14B Chat & 17.20  & \textbf{71.74 } & 55.06  & 21.00  & 18.78  & 23.82  & 17.75  & 42.50  \\
    Qwen 2.5 3B Chat & 16.30  & \textbf{64.48 } & 43.81  & 18.00  & 30.94  & 38.30  & 20.35  & 42.20  \\
    Qwen 2.5 14B Chat & 3.80  & 12.83  & 11.95  & 22.00  & 15.42  & 9.38  & 15.65  & \textbf{17.15 } \\
    \bottomrule
    \end{tabular}%
  }
  \caption{Add caption}
  \label{tab:effective}%
\end{table*}%

==> tables/effective_v2.tex <==
\begin{table*}[t]
  \centering
  \newcolumntype{C}{>{\centering\arraybackslash}p{9em}} 
  \renewcommand{\arraystretch}{.9} 

  \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{ASR_{tst}\uparrow} & \multicolumn{1}{c}{Direct Attack} & \multicolumn{1}{C}{Few-Shot} & \multicolumn{1}{C}{Imtate Learning} & \multicolumn{1}{C}{Reinforce Learning} & \multicolumn{1}{c}{\our{}} \\
    \midrule
    Vicuna 7B & 24.80  & 29.58  & 36.90  & 31.95  & \textbf{56.40}  \\
    Vicuna 13B & 16.60  & 20.80  & 36.08  & 17.80  & \textbf{55.35}  \\
    Llama 2 7B Chat & 0.45  & 6.84  & 6.67  & 0.50  & \textbf{13.50 } \\
    Llama 2 13B Chat & 1.30  & 5.88  & 6.80  & 2.05  & \textbf{11.00}  \\
    Llama 3 8B Instruct & 3.20  & 9.42  & 7.18  & 14.55  & \textbf{15.00 } \\
    Mistral 7B Instruct & 48.50  & 51.54  & 54.88  & 44.20  & \textbf{52.65}  \\
    Yi 6B Chat & 13.45  & 36.00  & 42.29  & 33.80  & \textbf{52.50}  \\
    Yi 9B Chat & 16.75  & 28.06  & 34.23  & 39.75  & \textbf{49.20}  \\
    Gemma 2 2b Instruct & 2.05  & 5.64  & 7.49  & 6.15  & \textbf{48.15}  \\
    Gemma 2 9b Instruct & 1.55  & 3.74  & 6.63  & \textbf{44.85}  & 44.80  \\
    R2D2  & 1.70  & 27.18  & \textbf{24.24}  & 8.60  & 12.45  \\
    Qwen 1.5 4B Chat & 12.50  & 27.24  & 18.52  & 17.45  & \textbf{51.30}  \\
    Qwen 1.5 7B Chat & 21.70  & 23.80  & 18.82  & 32.60  & \textbf{49.85}  \\
    Qwen 1.5 14B Chat & 17.20  & 18.78  & 23.82  & 17.75  & \textbf{42.50}  \\
    Qwen 2.5 3B Chat & 16.30  & 30.94  & 38.30  & 20.35  & \textbf{42.20}  \\
    Qwen 2.5 14B Chat & 3.80  & 15.42  & 9.38  & 15.65  & \textbf{17.15 } \\
    \bottomrule
    \end{tabular}%
  }
  \caption{Add caption}
  \label{tab:effective}%
\end{table*}%

==> tables/inverse.tex <==
% Table generated by Excel2LaTeX from sheet 'first'
\begin{table}[t]
  \centering
    % \renewcommand{\arraystretch}{1.4} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
       \multicolumn{1}{c}{ \textbf{ASR_{tst}}\uparrow}   & TM^{1}    & TM^{2}    & TM^{3}    & TM^{4}    & TM^{5}    & TM^{6} \\
    \midrule
    Qwen 1.5 14B  & 34.50  & 40.88  & 42.11  & \textbf{42.50 } & 32.45  & 27.62  \\
    Qwen 1.5 4B  & 40.59  & 51.15  & 49.54  & 51.04  & \textbf{51.30 } & 45.68  \\
    Qwen 2.5 14B  & 15.66  & 15.99  & 15.35  & 16.84  & \textbf{17.15 } & 11.14  \\
    Llama 3 8B  & 14.88  & \textbf{15.00 } & 12.72  & 12.98  & 13.08  & 14.59  \\
    Llama 2 7B  & 1.97  & 9.18  & \textbf{13.50 } & 13.04  & 11.29  & 9.97  \\
    Qwen 1.5 14B  & 34.50  & 40.88  & 42.11  & \textbf{42.50 } & 32.45  & 27.62  \\
    
    
    \bottomrule
    \end{tabular}%
    }
  \caption{The ASR$_{tst}$ achieved by using different intermediate models as the degrade model for reward shaping.}
  \label{tab:firstinverse}%
\end{table}%
\vspace{-0.3cm}

